Strategic Classification under Unknown Personalized Manipulation

We study the fundamental mistake bound and sample complexity in the strategic classification, where agents can strategically manipulate their feature vector up to an extent in order to be predicted as positive. For example, given a classifier determining college admission, student candidates may try to take easier classes to improve their GPA, retake SAT and change schools in an effort to fool the classifier. Ball manipulations are a widely studied class of manipulations in the literature, where agents can modify their feature vector within a bounded radius ball. Unlike most prior work, our work considers manipulations to be personalized, meaning that agents can have different levels of manipulation abilities (e.g., varying radii for ball manipulations), and unknown to the learner. We formalize the learning problem in an interaction model where the learner first deploys a classifier and the agent manipulates the feature vector within their manipulation set to game the deployed classifier. We investigate various scenarios in terms of the information available to the learner during the interaction, such as observing the original feature vector before or after deployment, observing the manipulated feature vector, or not seeing either the original or the manipulated feature vector. We begin by providing online mistake bounds and PAC sample complexity in these scenarios for ball manipulations. We also explore non-ball manipulations and show that, even in the simplest scenario where both the original and the manipulated feature vectors are revealed, the mistake bounds and sample complexity are lower bounded by $\Omega(|H|)$ when the target function belongs to a known class $H$.

==> src/extra_related_work.tex <==
\section{Additional Related Work}\label{app:relatedwork}
There has been a lot of research on various other issues and models in strategic classification. 
Beyond sample complexity, \cite{hu2019disparate,milli2019social} focused on other social objectives, such as social burden and fairness. 
Recent works also explored different models of agent behavior, including
proactive agents~\cite{zrnic2021leads}, non-myopic agents~\citep{haghtalab2022learning} and noisy agents~\citep{jagadeesan2021alternative}.
\cite{ahmadi2023fundamental} considers two agent models of randomized learners: a randomized algorithm model where the agents respond to the realization, and a fractional classifier model where agents respond to the expectation, and our model corresponds to the randomized algorithm model.
Additionally, there is also a line of research on agents interested in improving their qualifications instead of gaming~\citep{kleinberg2020classifiers, haghtalab2020maximizing,ahmadi2022classification}.
Strategic interactions in the regression setting have also been studied~\citep{bechavod2021gaming}.

Beyond strategic classification, there is a more general research area of learning using data from strategic sources, such as a single data generation player who manipulates the data distribution~\citep{bruckner2011stackelberg,dalvi2004adversarial}. Adversarial perturbations can be viewed as another type of strategic source~\citep{montasser2019vc}.
